Robust Linear Regression Analysis - A Greedy Approach

The task of robust linear estimation in the presence of outliers is of particular importance in signal processing, statistics and machine learning. Although the problem has been stated a few decades ago and solved using classical (considered nowadays) methods, recently it has attracted more attention in the context of sparse modeling, where several notable contributions have been made. In the present manuscript, a new approach is considered in the framework of greedy algorithms. The noise is split into two components: a) the inlier bounded noise and b) the outliers, which are explicitly modeled by employing sparsity arguments. Based on this scheme, a novel efficient algorithm (Greedy Algorithm for Robust Denoising - GARD), is derived. GARD alternates between a least square optimization criterion and an Orthogonal Matching Pursuit (OMP) selection step that identifies the outliers. The case where only outliers are present has been studied separately, where bounds on the \textit{Restricted Isometry Property} guarantee that the recovery of the signal via GARD is exact. Moreover, theoretical results concerning convergence as well as the derivation of error bounds in the case of additional bounded noise are discussed. Finally, we provide extensive simulations, which demonstrate the comparative advantages of the new technique.

==> Geo_Library.bbl.tex <==
@Book{smolalearningwithKer,
  title={Learning with Kernels}, 
  author={Smola, Alex J. and Sch{\"o}lkopf, Bernhard},
  year={2002},
  publisher={The MIT Press}
}

@book{bjorck1996numerical,
  title={Numerical methods for least squares problems},
  author={Bj{\"o}rck, {\AA}ke},
  number={51},
  year={1996},
  publisher={Society for Industrial and Applied Mathematics}
}

@book{theodoridis2010introduction,
  title={Introduction to Pattern Recognition: A Matlab Approach},
  author={Theodoridis, Sergios and Pikrakis, Aggelos and Koutroumbas, Konstantinos and Cavouras, Dionisis},
  year={2010},
  publisher={Academic Press}
}

@book{mallat2008wavelet,
  title={A wavelet tour of signal processing: the sparse way},
  author={Mallat, Stephane},
  year={2008},
  publisher={Academic press}
}

@article{mateos2012robust,
  title={Robust nonparametric regression via sparsity control with application to load curve data cleansing},
  author={Mateos, Gonzalo and Giannakis, Georgios B.},
  journal={Signal Processing, IEEE Transactions on},
  volume={60},
  number={4},
  pages={1571--1584},
  year={2012},
  publisher={IEEE}
}

@article{Peirce,
  author = 	 {Benjamin Peirce},
  title = 	 {Criterion for the Rejection of Doubtful Observations},
  journal = 	 {Astronomical Journal II and Errata},
  year = 	 {1852},
  volume = 	 {Astronomical Journal II 45},
}

@article{Grubbs,
  author = 	 {Grubbs, F.~E.},
  title = 	 {Procedures for detecting outlying observations in samples},
  journal = 	 {Technometrics},
  year = 	 {1969},
  volume = 	 {11},
  number={1},
  pages={1--21}
}

@article{brucksteindonohoeladsparse,
  title = {From sparse solutions of systems of equations to sparse modeling of signals and images},
  author = {Bruckstein, Alfred M. and Donoho, David L. and Elad, Michael},
  journal={SIAM review},
  volume={51},
  number={1},
  pages={34--81},
  year={2009},
  publisher={SIAM}
}

@article{tropp2004greed,
  title={Greed is good: Algorithmic results for sparse approximation},
  author={Tropp, Joel A},
  journal={Information Theory, IEEE Transactions on},
  volume={50},
  number={10},
  pages={2231--2242},
  year={2004},
  publisher={IEEE}
}

@article{tropp2007signal,
  title={Signal recovery from random measurements via orthogonal matching pursuit},
  author={Tropp, Joel A and Gilbert, Anna C},
  journal={Information Theory, IEEE Transactions on},
  volume={53},
  number={12},
  pages={4655--4666},
  year={2007},
  publisher={IEEE}
}

@article{needell2009uniform,
  title={Uniform uncertainty principle and signal recovery via regularized orthogonal matching pursuit},
  author={Needell, Deanna and Vershynin, Roman},
  journal={Foundations of computational mathematics},
  volume={9},
  number={3},
  pages={317--334},
  year={2009},
  publisher={Springer}
}

@article{blumensath2007difference,
  title={On the difference between orthogonal matching pursuit and orthogonal least squares},
  author={Blumensath, Thomas and Davies, Mike E},
  year={2007},
  publisher={TechReport}
}

@inproceedings{mitra2010robust,
  title={Robust RVM regression using sparse outlier model},
  author={Mitra, Kaushik and Veeraraghavan, Ashok and Chellappa, Rama},
  booktitle={Computer Vision and Pattern Recognition (CVPR), Conference on},
  pages={1887--1894},
  year={2010},
  organization={IEEE}
}

@inproceedings{giannakis2011uspacor,
  title={USPACOR: Universal sparsity-controlling outlier rejection},
  author={Giannakis, GB and Mateos, G and Farahmand, S and Kekatos, V and Zhu, H},
  booktitle={Acoustics, Speech and Signal Processing (ICASSP), 2011 IEEE International Conference on},
  pages={1952--1955},
  year={2011},
  organization={IEEE}
}

@book{gander1978linear,
  title={On the linear least squares problem with a quadratic constraint},
  author={Gander, Walter},
  year={1978},
  publisher={Computer Science Department, Stanford University}
}

@article{gander1980least,
  title={Least squares with a quadratic constraint},
  author={Gander, Walter},
  journal={Numerische Mathematik},
  volume={36},
  number={3},
  pages={291--307},
  year={1980},
  publisher={Springer}
}

@article{candes2005decoding,
  title={Decoding by linear programming},
  author={Candes, Emmanuel J and Tao, Terence},
  journal={Information Theory, IEEE Transactions on},
  volume={51},
  number={12},
  pages={4203--4215},
  year={2005},
  publisher={IEEE}
}

@article{rojas2002trust,
  title={A trust-region approach to the regularization of large-scale discrete forms of ill-posed problems},
  author={Rojas, Marielba and Sorensen, Danny C},
  journal={SIAM Journal on Scientific Computing},
  volume={23},
  number={6},
  pages={1842--1860},
  year={2002},
  publisher={SIAM}
}

@article{slavakis2009adaptive,
  title={Adaptive constrained learning in reproducing kernel Hilbert spaces: the robust beamforming case},
  author={Slavakis, Konstantinos and Theodoridis, Sergios and Yamada, Isao},
  journal={Signal Processing, IEEE Transactions on},
  volume={57},
  number={12},
  pages={4744--4764},
  year={2009},
  publisher={IEEE}
}

@article{donoho2006stable,
  title={Stable recovery of sparse overcomplete representations in the presence of noise},
  author={Donoho, David Leigh and Elad, Michael and Temlyakov, Vladimir N},
  journal={Information Theory, IEEE Transactions on},
  volume={52},
  number={1},
  pages={6--18},
  year={2006},
  publisher={IEEE}
}

@article{fuchs2005recovery,
  title={Recovery of exact sparse representations in the presence of bounded noise},
  author={Fuchs, Jean-Jacques},
  journal={Information Theory, IEEE Transactions on},
  volume={51},
  number={10},
  pages={3601--3608},
  year={2005},
  publisher={IEEE}
}

@article{gribonval2006exponential,
  title={On the exponential convergence of matching pursuits in quasi-incoherent dictionaries},
  author={Gribonval, R{\'e}mi and Vandergheynst, Pierre},
  journal={Information Theory, IEEE Transactions on},
  volume={52},
  number={1},
  pages={255--261},
  year={2006},
  publisher={IEEE}
}

@article{wohlberg2003noise,
  title={Noise sensitivity of sparse signal representations: Reconstruction error bounds for the inverse problem},
  author={Wohlberg, Brendt},
  journal={Signal Processing, IEEE Transactions on},
  volume={51},
  number={12},
  pages={3053--3060},
  year={2003},
  publisher={IEEE}
}

@inproceedings{li2011fast,
  title={Fast kernel sparse representation},
  author={Li, Hanxi and Gao, Yongsheng and Sun, Jun},
  booktitle={Digital Image Computing Techniques and Applications (DICTA), 2011 International Conference on},
  pages={72--77},
  year={2011},
  organization={IEEE}
}

@article{takeda2007kernel,
  title={Kernel regression for image processing and reconstruction},
  author={Takeda, Hiroyuki and Farsiu, Sina and Milanfar, Peyman},
  journal={Image Processing, IEEE Transactions on},
  volume={16},
  number={2},
  pages={349--366},
  year={2007},
  publisher={IEEE}
}

@article{durand2003reconstruction,
  title={Reconstruction of wavelet coefficients using total variation minimization},
  author={Durand, Sylvain and Froment, Jacques},
  journal={SIAM Journal on Scientific computing},
  volume={24},
  number={5},
  pages={1754--1767},
  year={2003},
  publisher={SIAM}
}

@article{combettes2004image,
  title={Image restoration subject to a total variation constraint},
  author={Combettes, Patrick L and Pesquet, J-C},
  journal={Image Processing, IEEE Transactions on},
  volume={13},
  number={9},
  pages={1213--1222},
  year={2004},
  publisher={IEEE}
}

@article{soussen2013joint,
  title={Joint k-step analysis of orthogonal matching pursuit and orthogonal least squares},
  author={Soussen, Charles and Gribonval, R{\'e}mi and Idier, J{\'e}r{\^o}me and Herzet, C{\'e}dric},
  year={2013},
  publisher={IEEE}
}

@inproceedings{sturm2011cyclic,
  title={Cyclic pure greedy algorithms for recovering compressively sampled sparse signals},
  author={Sturm, Bob L and Christensen, Mads G and Gribonval, R{\'e}mi},
  booktitle={Signals, Systems and Computers (ASILOMAR), 2011 Conference Record of the Forty Fifth Asilomar Conference on},
  pages={1143--1147},
  year={2011},
  organization={IEEE}
}

@inproceedings{pati1993orthogonal,
  title={Orthogonal matching pursuit: Recursive function approximation with applications to wavelet decomposition},
  author={Pati, Yagyensh Chandra and Rezaiifar, Ramin and Krishnaprasad, PS},
  booktitle={Signals, Systems and Computers, Conference Record of The Twenty-Seventh Asilomar Conference on},
  pages={40--44},
  year={1993},
  organization={IEEE}
}

@book{theodoridis2008koutroumbas,
  title={Pattern Recognition, 4th Edition},
  author={Theodoridis, Sergios and Koutroumbas, Konstantinos},
  year={2008},
  publisher={Academic press}
}

@article{bouboulis2010adaptive,
  title={Adaptive kernel-based image denoising employing semi-parametric regularization},
  author={Bouboulis, Pantelis and Slavakis, Konstantinos and Theodoridis, Sergios},
  journal={Image Processing, IEEE Transactions on},
  volume={19},
  number={6},
  pages={1465--1479},
  year={2010},
  publisher={IEEE}
}

@inproceedings{sturm2012comparison,
  title={Comparison of orthogonal matching pursuit implementations},
  author={Sturm, Bob L and Christensen, Mads Graesboll},
  booktitle={Signal Processing Conference (EUSIPCO), Proceedings of the 20th European},
  pages={220--224},
  year={2012},
  organization={IEEE}
}

@article{mitra2013analysis,
  title={Analysis of Sparse Regularization Based Robust Regression Approaches},
  author={Mitra, Kaushik and Veeraraghavan, Ashok and Chellappa, Rama},
  journal={Signal Processing, IEEE Transactions on},
  volume={61},
  number={5},
  pages={1249--1257},
  year={2013},
  publisher={IEEE}
}

@inproceedings{theodoridisrobust,
  title={ROBUST KERNEL-BASED REGRESSION USING ORTHOGONAL MATCHING PURSUIT},
  author={Papageorgiou, George and Bouboulis Pantelis and Theodoridis, Sergios},
  booktitle={International Workshop on
Machine Learning for Signal Processing (MLSP2013)},
volume={61},
number={5},
pages={1249--1257}, 
year={2013},
publisher={IEEE}
}

@inproceedings{razavi2012robust,
  title={Robust greedy algorithms for compressed sensing},
  author={Razavi, S Alireza and Ollila, Esa and Koivunen, Visa},
  booktitle={Signal Processing Conference (EUSIPCO), Proceedings of the 20th European},
  pages={969--973},
  year={2012},
  organization={IEEE}
}

@article{lobo1998applications,
  title={Applications of second-order cone programming},
  author={Lobo, Miguel Sousa and Vandenberghe, Lieven and Boyd, Stephen and Lebret, Herv{\'e}},
  journal={Linear algebra and its applications},
  volume={284},
  year={1998},
  publisher={Elsevier}
}
% Robust statistics
@Book{huber1981wiley,
  title={Wiley Series in Probability and Mathematics Statistics},
  author={Huber, Peter J},
  year={1981},
  publisher={Wiley Online Library}
}

@book{maronna2006robust,
  title={Robust statistics},
  author={Maronna, Ricardo A and Martin, R Douglas and Yohai, Victor J},
  year={2006},
  publisher={J. Wiley}
}

@book{rousseeuw2005robust,
  title={Robust regression and outlier detection},
  author={Rousseeuw, Peter J and Leroy, Annick M},
  volume={589},
  year={2005},
  publisher={John Wiley \& Sons}
}


@inproceedings{razavi2012robust,
  title={Robust greedy algorithms for compressed sensing},
  author={Razavi, S Alireza and Ollila, Esa and Koivunen, Visa},
  booktitle={Signal Processing Conference (EUSIPCO), 2012 Proceedings of the 20th European},
  pages={969--973},
  year={2012},
  organization={IEEE}
}

@article{huber19721972,
  title={The 1972 wald lecture robust statistics: A review},
  author={Huber, Peter J},
  journal={The Annals of Mathematical Statistics},
  pages={1041--1067},
  year={1972},
  publisher={JSTOR}
}
@article{rousseeuw1990unmasking,
  title={Unmasking multivariate outliers and leverage points},
  author={Rousseeuw, Peter J and Van Zomeren, Bert C},
  journal={Journal of the American Statistical Association},
  volume={85},
  number={411},
  pages={633--639},
  year={1990},
  publisher={Taylor \& Francis}
}
@article{leroy1987robust,
  title={Robust regression and outlier detection},
  author={Leroy, Annick M and Rousseeuw, Peter J},
  journal={J. Wiley\&Sons, New York},
  year={1987}
}

@article{boyd2011distributed,
  title={Distributed optimization and statistical learning via the alternating direction method of multipliers},
  author={Boyd, Stephen and Parikh, Neal and Chu, Eric and Peleato, Borja and Eckstein, Jonathan},
  journal={Foundations and Trends{\textregistered} in Machine Learning},
  volume={3},
  number={1},
  pages={1--122},
  year={2011},
  publisher={Now Publishers Inc.}
}

@inproceedings{boyd2011alternating,
  title={Alternating Direction Method of Multipliers},
  author={Boyd, Stephen},
  booktitle={Talk at NIPS Workshop on Optimization and Machine Learning},
  year={2011}
}


@article{chen1998atomic,
  title={Atomic decomposition by basis pursuit},
  author={Chen, Scott Shaobing and Donoho, David L and Saunders, Michael A},
  journal={SIAM journal on scientific computing},
  volume={20},
  number={1},
  pages={33--61},
  year={1998},
  publisher={SIAM}
}

@article{candes2006stable,
  title={Stable signal recovery from incomplete and inaccurate measurements},
  author={Candes, Emmanuel J and Romberg, Justin K and Tao, Terence},
  journal={Communications on pure and applied mathematics},
  volume={59},
  number={8},
  pages={1207--1223},
  year={2006},
  publisher={Wiley Online Library}
}

@article{lustig2007sparse,
  title={Sparse MRI: The application of compressed sensing for rapid MR imaging},
  author={Lustig, Michael and Donoho, David and Pauly, John M},
  journal={Magnetic resonance in medicine},
  volume={58},
  number={6},
  pages={1182--1195},
  year={2007},
  publisher={Wiley Online Library}
}

@article{candes2006robust,
  title={Robust uncertainty principles: Exact signal reconstruction from highly incomplete frequency information},
  author={Cand{\`e}s, Emmanuel J and Romberg, Justin and Tao, Terence},
  journal={Information Theory, IEEE Transactions on},
  volume={52},
  number={2},
  pages={489--509},
  year={2006},
  publisher={IEEE}
}

@article{tibshirani1996regression,
  title={Regression shrinkage and selection via the lasso},
  author={Tibshirani, Robert},
  journal={Journal of the Royal Statistical Society. Series B (Methodological)},
  pages={267--288},
  year={1996},
  publisher={JSTOR}
}

@book{boyd2004convex,
  title={Convex optimization},
  author={Boyd, Stephen P and Vandenberghe, Lieven},
  year={2004},
  publisher={Cambridge university press}
}

@article{davis1997adaptive,
  title={Adaptive greedy approximations},
  author={Davis, Geoff and Mallat, Stephane and Avellaneda, Marco},
  journal={Constructive approximation},
  volume={13},
  number={1},
  pages={57--98},
  year={1997},
  publisher={Springer}
}

@article{mallat1993matching,
  title={Matching pursuits with time-frequency dictionaries},
  author={Mallat, St{\'e}phane G and Zhang, Zhifeng},
  journal={Signal Processing, IEEE Transactions on},
  volume={41},
  number={12},
  pages={3397--3415},
  year={1993},
  publisher={IEEE}
}

% SBL
@article{tipping2001sparse,
  title={Sparse Bayesian learning and the relevance vector machine},
  author={Tipping, Michael E},
  journal={The journal of machine learning research},
  volume={1},
  pages={211--244},
  year={2001},
  publisher={JMLR. org}
}

@article{wipf2004sparse,
  title={Sparse Bayesian learning for basis selection},
  author={Wipf, David P and Rao, Bhaskar D},
  journal={Signal Processing, IEEE Transactions on},
  volume={52},
  number={8},
  pages={2153--2164},
  year={2004},
  publisher={IEEE}
}

@inproceedings{jin2010algorithms,
  title={Algorithms for robust linear regression by exploiting the connection to sparse signal recovery},
  author={Jin, Yuzhe and Rao, Bhaskar D},
  booktitle={Acoustics Speech and Signal Processing (ICASSP), International Conference on},
  pages={3830--3833},
  year={2010},
  organization={IEEE}
}
% Outliers
@article{grubbs1969procedures,
  title={Procedures for detecting outlying observations in samples},
  author={Grubbs, Frank E},
  journal={Technometrics},
  volume={11},
  number={1},
  pages={1--21},
  year={1969},
  publisher={Taylor \& Francis}
}

@article{dixon1950analysis,
  title={Analysis of extreme values},
  author={Dixon, Wilfred J and others},
  journal={The Annals of Mathematical Statistics},
  volume={21},
  number={4},
  pages={488--506},
  year={1950},
  publisher={Institute of Mathematical Statistics}
}
% Breakdown point
@article{he1990breakdown,
  title={Breakdown robustness of tests},
  author={He, Xuming and Simpson, Douglas G and Portnoy, Stephen L},
  journal={Journal of the American Statistical Association},
  volume={85},
  number={410},
  pages={446--452},
  year={1990},
  publisher={Taylor \& Francis}
}

@article{fischler1981random,
  title={Random sample consensus: a paradigm for model fitting with applications to image analysis and automated cartography},
  author={Fischler, Martin A and Bolles, Robert C},
  journal={Communications of the ACM},
  volume={24},
  number={6},
  pages={381--395},
  year={1981},
  publisher={ACM}
}

@article{needell2010signal,
  title={Signal recovery from incomplete and inaccurate measurements via regularized orthogonal matching pursuit},
  author={Needell, Deanna and Vershynin, Roman},
  journal={Selected Topics in Signal Processing, IEEE Journal of},
  volume={4},
  number={2},
  pages={310--316},
  year={2010},
  publisher={IEEE}
}

@article{needell2009cosamp,
  title={CoSaMP: Iterative signal recovery from incomplete and inaccurate samples},
  author={Needell, Deanna and Tropp, Joel A},
  journal={Applied and Computational Harmonic Analysis},
  volume={26},
  number={3},
  pages={301--321},
  year={2009},
  publisher={Elsevier}
}

@article{tibshirani2013lasso,
  title={The lasso problem and uniqueness},
  author={Tibshirani, Ryan J and others},
  journal={Electronic Journal of Statistics},
  volume={7},
  pages={1456--1490},
  year={2013},
  publisher={Institute of Mathematical Statistics}
}

@book{zhang2006schur,
  title={The Schur complement and its applications},
  author={Zhang, Fuzhen},
  volume={4},
  year={2006},
  publisher={Springer}
}

@inproceedings{ramaswamy2000efficient,
  title={Efficient algorithms for mining outliers from large data sets},
  author={Ramaswamy, Sridhar and Rastogi, Rajeev and Shim, Kyuseok},
  booktitle={ACM SIGMOD Record},
  volume={29},
  number={2},
  pages={427--438},
  year={2000},
  organization={ACM}
}

@incollection{tang2002enhancing,
  title={Enhancing effectiveness of outlier detections for low density patterns},
  author={Tang, Jian and Chen, Zhixiang and Fu, Ada Wai-Chee and Cheung, David W},
  booktitle={Advances in Knowledge Discovery and Data Mining},
  pages={535--548},
  year={2002},
  publisher={Springer}
}

@inproceedings{chen2003modeling,
  title={Modeling and efficient mining of intentional knowledge of outliers},
  author={Chen, Zhixiang and Tang, Jian and Fu, Ada Wai-Chee},
  booktitle={Database Engineering and Applications Symposium, 2003. Proceedings. Seventh International},
  pages={44--53},
  year={2003},
  organization={IEEE}
}

@article{tang2007capabilities,
  title={Capabilities of outlier detection schemes in large datasets, framework and methodologies},
  author={Tang, Jian and Chen, Zhixiang and Fu, Ada Waichee and Cheung, David W},
  journal={Knowledge and Information Systems},
  volume={11},
  number={1},
  pages={45--84},
  year={2007},
  publisher={Springer}
}

@book{hawkins1980identification,
  title={Identification of outliers},
  author={Hawkins, Douglas M},
  volume={11},
  year={1980},
  publisher={Springer}
}

@book{barnett1994outliers,
  title={Outliers in statistical data},
  author={Barnett, Vic and Lewis, Toby},
  volume={3},
  year={1994},
  publisher={Wiley New York}
}

@book{moore1989introduction,
  title={Introduction to the Practice of Statistics.},
  author={Moore, David S and McCabe, George P},
  year={1989},
  publisher={WH Freeman/Times Books/Henry Holt \& Co}
}

@book{theodoridis2015machine_learning,
title={Machine Learning: A Bayesian and Optimization Perspective},
author={Theodoridis, Sergios},
year={2015},
publisher={Academic Press}
}

@article{peaceman1955numerical,
  title={The numerical solution of parabolic and elliptic differential equations},
  author={Peaceman, Donald W and Rachford, Jr, Henry H},
  journal={Journal of the Society for Industrial \& Applied Mathematics},
  volume={3},
  number={1},
  pages={28--41},
  year={1955},
  publisher={SIAM}
}

@article{douglas1955numerical,
  title={On the Numerical Integration of ∂\^{}2u∂x\^{}2+∂\^{}2u∂y\^{}2=∂u∂t by Implicit Methods},
  author={Douglas, Jr, Jim},
  journal={Journal of the Society for Industrial \& Applied Mathematics},
  volume={3},
  number={1},
  pages={42--65},
  year={1955},
  publisher={SIAM}
}

@article{donoho2003optimally,
  title={Optimally sparse representation in general (nonorthogonal) dictionaries via ℓ1 minimization},
  author={Donoho, David L and Elad, Michael},
  journal={Proceedings of the National Academy of Sciences},
  volume={100},
  number={5},
  pages={2197--2202},
  year={2003},
  publisher={National Acad Sciences}
}

@article{donoho2001uncertainty,
  title={Uncertainty principles and ideal atomic decomposition},
  author={Donoho, David L and Huo, Xiaoming},
  journal={Information Theory, IEEE Transactions on},
  volume={47},
  number={7},
  pages={2845--2862},
  year={2001},
  publisher={IEEE}
}













